MELOPPR: Software/Hardware Co-design for Memory-efficient Low-latency Personalized PageRank

Personalized PageRank (PPR) is a graph algorithm that evaluates the importance of the surrounding nodes from a source node. Widely used in social network related applications such as recommender systems, PPR requires real-time responses (latency) for a better user experience. Existing works either focus on algorithmic optimization for improving precision while neglecting hardware implementations or focus on distributed global graph processing on large-scale systems for improving throughput rather than response time. Optimizing low-latency local PPR algorithm with a tight memory budget on edge devices remains unexplored. In this work, we propose a memory-efficient, low-latency PPR solution, namely MeLoPPR, with largely reduced memory requirement and a flexible trade-off between latency and precision. MeLoPPR is composed of stage decomposition and linear decomposition and exploits the node score sparsity: Through stage and linear decomposition, MeLoPPR breaks the computation on a large graph into a set of smaller sub-graphs, that significantly saves the computation memory; Through sparsity exploitation, MeLoPPR selectively chooses the sub-graphs that contribute the most to the precision to reduce the required computation. In addition, through software/hardware co-design, we propose a hardware implementation on a hybrid CPU and FPGA accelerating platform, that further speeds up the sub-graph computation. We evaluate the proposed MeLoPPR on memory-constrained devices including a personal laptop and Xilinx Kintex-7 KC705 FPGA using six real-world graphs. First, MeLoPPR demonstrates significant memory saving by 1.5x to 13.4x on CPU and 73x to 8699x on FPGA. Second, MeLoPPR allows flexible trade-offs between precision and execution time: when the precision is 80%, the speedup on CPU is up to 15x and up to 707x on FPGA; when the precision is around 90%, the speedup is up to 70x on FPGA.

==> fpga-friendly-push.tex <==

\section{fpga-friendly-push}
We are going to compute 
\begin{align}
    p_0 = \sum_{k=0}^\infty \gamma_k W^k s.
\end{align}
where $W=AD^{-1}$, $A$ is the adjacent matrix and $D$ is the diagonal degree matrix. For normalization, $\sum_{k=0}^\infty\gamma_k = 1$. 
We view the solution in the following way. $p$ is termed as the solution vector, intialized as all $0$'s. $r$ is termed as the residual vector, initialized as $s$. 

The essence of push algorithm is to iteratively push the mass from $r$ to $p$ so that $p$ will component-wisely monotonically increase to approximate $p_0$. Of course, during the procedure $r$ have to be maintained. The way to maintain $r$ is in general via calling diffusion. When $r$ goes to 0, $p$ goes to $p_0$. %Keep in mind that during the entire procedure $\sum_{v\in V} p(v) + \sum_{v\in V} r(v) = \sum_{v\in V} s(v) =  \sum_{v\in V} p_0(v)$.

 \textbf{Parallel + Large Memory:} First think about the case that if we do not have memory constraint but have a very powerful parallel computing unit, how can we do the push algorithm? In $k$th iteration, we do the following iterations $k=1,2,...,$ ($p^{(0)}= 0$, $r^{(0)}= s$, $\gamma^{(0)}= \gamma_0$). 
\begin{enumerate}
    \item $p^{(k)} \leftarrow p^{(k-1)} + \gamma^{(k-1)} r^{(k-1)}$.
    \item $r^{(k)} \leftarrow  (1-\gamma^{(k-1)}) Wr^{(k-1)} $.
    \item  $\gamma^{(k)}\leftarrow  \frac{\gamma_k\gamma^{(k-1)}}{\gamma_{k-1}(1-\gamma^{(k-1)})}$. 
\end{enumerate}
Then, we have 
\begin{align*}
    \gamma^{(k)} = \frac{\gamma_k}{\sum_{i=k}^\infty \gamma_i}.  
\end{align*}
\begin{align*}
    r^{(k)}& = \prod_{i=0}^{k-1} (1-\gamma^{(i)}) Wr^{(0)} = (\sum_{i=k}^\infty\gamma_{i}) W^k s.  
\end{align*}
\begin{align*}
    p^{(k)}& = p^{(0)} + \sum_{i=1}^k \gamma^{(i-1)} r^{(i-1)} =  \sum_{i=0}^{k-1}  \gamma_{i} W^{i} s. % \gamma^{(0)}r^{(0)}+ \sum_{i=2}^k \gamma^{(i-1)} (\prod_{j=0}^{i-2} \gamma^{(j)} Wr^{(0)}) \\
    %&= \gamma_0s+  \sum_{i=2}^k  (\prod_{j=0}^{i-1} \gamma^{(j)}) W^{i-1} s = \gamma_0s+  \sum_{i=2}^k  \gamma_{i-1} W^{i-1} s = \sum_{i=0}^{k-1}  \gamma_{i} W^{i} s.
\end{align*}
%\begin{align*}
%    r^{(k)}& = \prod_{i=0}^{k-1} \gamma^{(i)} Wr^{(0)} = \gamma_{k-1} W^k s.  
%\end{align*}
The above iteration makes error control via $\|p_0 - p^{(k)}\|_1 = \sum_{i=k}^{\infty} \gamma_i = \|r^{(k)}\|_1$. This procedure is friendly to the parallel system with large memory, because in each iteration, the steps (1) and (2) are nothing but vector-sum and sparse-matrix-vector-product that can be computed in a fully parallel way. 

\textbf{Non-parallel + Large Memory:} In the standard CPU platform, the general assumption is that the CPU platform is a non-parallel system with sufficient memory. Sufficient memory indicates that one may access any node and its neighbors in a arbitrary way without additional overhead. Non-parallelization indicates that one cannot perform matrix/vector operation simultaneously. These two properties induce another push procedure. We still have $p$ to record the solution vector and $r$ to record the residual. However, in a CPU platform, we will never perform the above vector/matrix operation any more. Instead, we will keep check the residual for each node $r(v)$, $v\in V$. As long as $r(v)$ is non-zero (for accurate PageRank) or large than certain threshold (for approximate PageRank), we will pick this node $v$ and push some mass like step (1) but we only update $p(v)$ based on $r(v)$ instead of the entire vector $p$. Then, we will revise the residual $r$ via step (2) but it only affects $r(v)$ and $r(u)$ ($u\in \mathcal{N}_v$). However, the selection of $v$ makes the update of $p$ and $r$ in a non-synchronized way for different nodes. Here non-synchronization means the components in $p$ and $r$ are not updated as above for each $k$ before going into the next $k+1$ iteration. This may not guarantee convergence in general. But if we just focus on standard PageRank ($\gamma_k = (1-\alpha)\alpha^k$), the coefficients in the previous algorithm $\gamma^{(k)} = 1-\alpha$ does not change with respect to $k$, which finally allows us to update each single node in a non-synchronized way and the procedure still convergences. Overall, we have the following algorithm: We initialize $p^{(0)}= 0$, $r^{(0)}= s$. We do the following iterations $k=1,2,...,$: Check if there is an $v$ such that $\frac{r(v)}{d(v)} \geq \epsilon$. If there is no such $v$, return $p^{(k)}$ (more sparse) or $p^{(k)} + (1-\alpha) r^{(k)}$ (denser but more accurate). Otherwise, 
\begin{enumerate}
    \item $p^{(k)}(v) \leftarrow p^{(k-1)}(v) +  (1-\alpha) r^{(k-1)}(v)$
    \item $r^{(k)}(v) \leftarrow 0$, $r^{(k)}(u) \leftarrow r^{(k-1)}(u) + \alpha r^{(k-1)}(v) $ for $u\in \mathcal{N}_v$. $r^{(k)}(w) \leftarrow r^{(k-1)}(w)$ for all $w\notin \{v\}\cup \mathcal{N}_v$.
\end{enumerate}
Steps (1) and (2) are both very local operations: step 1 changes one component; step 2 changes 1+$|\mathcal{N}_v|$ components. This favors non-parallel systems. 

The approximating error regarding each node $v$ can be viewed as $\frac{r(v)}{d(v)}$. But please keep in mind that $\frac{r(v)}{d(v)}$ is not proportional to the true error $(p_0(v) - p^{(k)}(v))/d(v)$. This is why in \cite{wang2019efficient}. But in general, it is good enough to control the error.   

\textbf{Parallel + Limited Memory:} This is the FPGA setting. This means that we are unable to access each node or the neighbors of a node in an arbitrary way. But we allow matrix/vector operation. The insight of the algorithm for this setting is in 2 folds. First, the push method will keep decreasing the error $\|r^{(k)}\|_1 = \|p_0 - p^{(k)}\|_1$. Therefore, as along as we do more push, our results are always more accurate. Second, the push method of the standard PageRank allows for non-synchronized iterations while keeping converging (as illustrated in the CPU platform). This means when we extract a subgraph and load it into the memory, we can first do an arbitrary number of push operations over this subgraph, which still guarantees convergence. Due to the benefit of parallel computing unit, we may do push operation over this subgraph in a parallel and extremely efficient way. This gives us the algorithm. Here, we provide two algorithms due to the tradeoff in practice.

\textbf{Alg1:} We initialize $p^{(0)}= 0$, $r^{(0)}= s$. We do the following iterations $k=1,2,...,$ (outerloop-CPU). Check if there is an $v$ such that $\frac{r(v)}{d(v)} \geq \epsilon$. If there is no such $v$, return $p^{(k)}$ (more sparse), $p^{(k)} + (1-\alpha) r^{(k)}$ (denser but more accurate) or top-K in $p^{(k)} + (1-\alpha) r^{(k)}$ (for community detection). Otherwise, exact a subgraph $G_v$ around $v$. Initialize $x^{(0)}=0$. $y^{(0)}= r^{(k-1)}(G_v)$. $z^{(0)} = 0$. In the parallel unit, perform for $k'=1, 2,..., K_1$  ($K_1$ is large enough to guarantee $\|y^{(K_1)}\|_1$ is small) (innerloop-FPGA) %until $\|r^{(k, k')}\|_1<\epsilon_1$ 
 \begin{enumerate}
    \item $x^{(k')}\leftarrow x^{(k'-1)}+  (1-\alpha) y^{(k'-1)}$
    \item     $z^{(k')}\leftarrow z^{(k-1)} + \alpha w_{out, G_v} \odot y^{(k'-1)}$
    \item $y^{(k')} \leftarrow \alpha W_{G_v, G_v} y^{(k'-1)}$. .
\end{enumerate}
Here $w_{out, G_v}$ is a vector where each component corresponds to a node in $G_v$. For $u\in G_v$, $w_{out, G_v}(u) = 1$ if $u$ has an edge out of $G_v$ and otherwise $0$. 
%where $d_{out, G_v}(u)$ is $d(u) - d_{G_v}(u)$ and $d_{G_v}(u)$ is the number of edges of $u$ in $G_u$. 
After this, do $p^{(k)}(G_v) \leftarrow p^{(k-1)}(G_v) + x^{(K_1)}$ and $r^{(k)}(G_v)\leftarrow y^{(K_1)}$. For for each $u\in G_v$, $z^{(K_1)}(u) >0$, for each $q\in \mathcal{N}_u$ and $q\notin G_v$, $r^{(k)}(q) \leftarrow r^{(k-1)}(q) + \frac{z^{(K_1)}(u)}{d(u)}$.

%In the CPU side, do: for each $u\in G_v$, $q(u) >0$, $r$





\textcolor{red}{Pan: To clarify coefficients + sampling
\textbf{Alg2:} We initialize $p^{(0)}= 0$, $r^{(0)}= s$. We do the following iterations $k=1,2,...,$ (outerloop-CPU). Check if there is an $v$ such that $\frac{r(v)}{d(v)} \geq \epsilon$. If there is no such $v$, return $p^{(k)}$ (more sparse), $p^{(k)} + (1-\alpha) r^{(k)}$ (denser but more accurate) or top-K in $p^{(k)} + (1-\alpha) r^{(k)}$ (for community detection). Otherwise, extract the subgraph $G_{v}$ with in $q$-hop of $v$. Let $\partial G_v$ be the set of nodes in the exactly $q$-hop neighbor of $v$. For a node $u\in \partial G_v$, denote the number of edges of $u$ that are out of $G_{v}$ as $d_out(u)$. We randomly sample $cd_out(u)$. Initialize $x^{(0)}=0$. $y^{(0)}= r^{(k-1)}(G_{v,q})$. $z^{(0)} = 0$. In the parallel unit, perform for $k'=1, 2,..., K_1$  ($K_1$ is large enough to guarantee $\|y^{(K_1)}\|_1$ is small) (innerloop-FPGA) %until $\|r^{(k, k')}\|_1<\epsilon_1$ 
 \begin{enumerate}
    \item $x^{(k')}\leftarrow x^{(k'-1)}+  (1-\alpha) y^{(k'-1)}$
    \item $y^{(k')} \leftarrow y^{(k'-1)}  + \alpha W_{G_{v,q}, G_{v, q-1}} y^{(k'-1)}(G_{v, q-1})$. 
\end{enumerate}
Here $w_{out, G_v}$ is a vector where each component corresponds to a node in $G_v$. For $u\in G_v$, $w_{out, G_v}(u) = 1$ if $u$ has an edge out of $G_v$ and otherwise $0$. 
where $d_{out, G_v}(u)$ is $d(u) - d_{G_v}(u)$ and $d_{G_v}(u)$ is the number of edges of $u$ in $G_u$. 
After this, do $p^{(k)}(G_v) \leftarrow p^{(k-1)}(G_v) + x^{(K_1)}$ and $r^{(k)}(G_v)\leftarrow y^{(K_1)}$. For for each $u\in G_v$, $z^{(K_1)}(u) >0$, for each $q\in \mathcal{N}_u$ and $q\notin G_v$, $r^{(k)}(q) \leftarrow r^{(k-1)}(q) + \frac{z^{(K_1)}(u)}{d(u)}$.
}






%This is the algorithm:
%To take case of the non-synchronized $\gamma^{(k)}$ in this case, we assign a vector $\Gamma \in \mathbb{R}^{V}$ to record these weights.

%The error regarding each node $v$ can be viewed as $\frac{\sum_{i=k}^{\infty} \gamma_i}{\gamma_{k-1}} r(v)$. But please keep in mind that $r(v)$ is not proportional to $(p_0(v) - p^{(k)}(v))$. This is why in \cite{wang2019efficient}.
